Out-of-Vocabulary Entities in Link Prediction

Knowledge graph embedding techniques are key to making knowledge graphs amenable to the plethora of machine learning approaches based on vector representations. Link prediction is often used as a proxy to evaluate the quality of these embeddings. Given that the creation of benchmarks for link prediction is a time-consuming endeavor, most work on the subject matter uses only a few benchmarks. As benchmarks are crucial for the fair comparison of algorithms, ensuring their quality is tantamount to providing a solid ground for developing better solutions to link prediction and ipso facto embedding knowledge graphs. First studies of benchmarks pointed to limitations pertaining to information leaking from the development to the test fragments of some benchmark datasets. We spotted a further common limitation of three of the benchmarks commonly used for evaluating link prediction approaches: out-of-vocabulary entities in the test and validation sets. We provide an implementation of an approach for spotting and removing such entities and provide corrected versions of the datasets WN18RR, FB15K-237, and YAGO3-10. Our experiments on the corrected versions of WN18RR, FB15K-237, and YAGO3-10 suggest that the measured performance of state-of-the-art approaches is altered significantly with p-values <1%, <1.4%, and <1%, respectively. Overall, state-of-the-art approaches gain on average absolute $3.29 \pm 0.24\%$ in all metrics on WN18RR. This means that some of the conclusions achieved in previous works might need to be revisited. We provide an open-source implementation of our experiments and corrected datasets at at https://github.com/dice-group/OOV-In-Link-Prediction.

==> tables/table-scoring-functions.tex <==
\begin{table*}[tb]
\centering
  \caption{State-of-the-art \ac{KGE} models with training strategies. $\emb{}$ denotes embeddings, $\overline{\emb{}} \in \ComplexNumbers$ corresponds to the complex conjugate of $\emb{.}$. $\ast$ denotes a convolution operation with $\omega$ kernel. $f$ denotes rectified linear unit function. $\bigstar,\otimes, \circ, \cdot$ denotes the Octonion, Hamilton, the Hadamard and an inner product, respectively.
  $\triangleleft$ denotes unit normalization.
  $\ConvolutionWithProjection(.,.)$ corresponds to a convolution operation followed by linear transformation. $\langle x,y,z \rangle = \sum_{i} x_{i} y_{i} z_{i}$ denotes the trilinear inner product. In ConvE, the reshaping operation is omitted. The tensor product along the $n$-th mode is denoted by $\times_n$ and the core tensor is represented by $\mathcal{W}$. MSE, MR, BCE and CE denote mean squared error, margin ranking, binary cross entropy and cross entropy loss functions. NegSamp and AdvNegSamp stand for negative sampling and adversarial sampling.}
  \label{table:models}
%\scalebox{0.90}{%
%\footnotesize
\fontsize{8}{9.5}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l@{}ccccc@{}c@{}}
  \toprule
  Model & Scoring Function & VectorSpace & Loss & Training & Optimizer & Regularizer\\
  \midrule
   RESCAL~\citeyearpar{nickel2011three}          & $\emb{h}\cdot\mathcal{W}_r \cdot\emb{t}$                                                                       & $\emb{h}, \emb{t} \in \RealNumbers$           & MSE & Full    & ALS     & L2 \\
   DistMult~\citeyearpar{yang2015embedding}      & $\langle \emb{h}, \emb{r}, \emb{t} \rangle$                                                                    & $\emb{h},\emb{r},\emb{t} \in \RealNumbers$    & MR  & NegSamp & Adagrad & Weighted L2 \\
   ComplEx~\citeyearpar{trouillon2016complex}    & $\real(\langle \emb{h}, \emb{r}, \overline{ \emb{t}} \rangle)$                                                 & $\emb{h},\emb{r},\emb{t} \in \ComplexNumbers$ & BCE & NegSamp & Adagrad & Weighted L2 \\
   ConvE~\citeyearpar{dettmers2018convolutional} & $f ( \vect ( f ([ \emb{h} ; \emb{r} ] \ast \omega )) \lt ) \cdot \emb{t}$                                      & $\emb{h},\emb{r},\emb{t} \in \RealNumbers$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   TuckER~\citeyearpar{balavzevic2019tucker}     & $\mathcal{W} \times_1 \emb{h} \times_2 \emb{r} \times_3 \emb{t}$                                               & $\emb{h},\emb{r},\emb{t} \in \RealNumbers$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   RotatE~\citeyearpar{sun2019rotate}            &  -$\parallel \emb{h} \circ \emb{r} - \emb{t}\parallel$                                                         & $\emb{h},\emb{r},\emb{t} \in \ComplexNumbers$
   &CE&AdvNegSamp&Adam&-\\                                                                     
   QuatE~\citeyearpar{zhang2019quaternion}       & $ \emb{h}\otimes \emb{r}^{\triangleleft} \cdot\emb{t}$                                                         & $\emb{h},\emb{r},\emb{t} \in \Quaternions$    & CE  & AdvNegSamp & Adagrad    & Weighted L2 \\
%   QuaR~\citeyearpar{chen2020quaternion}       & $\parallel \emb{h} \circ \emb{r} - \emb{t}\parallel$                                                         & $\emb{h},\emb{r},\emb{t} \in \Quaternions$    & CE  &NegSamp & Adam   & - \\
%   OctonionE~\citeyearpar{zhang2019quaternion}   & $ \emb{h}\bigstar \emb{r}^{\triangleleft} \cdot\emb{t}$                                                        & $\emb{h},\emb{r},\emb{t} \in \Octonions$      & CE  & AdvNegSamp & Adagrad    & Weighted L2 \\
   \midrule
   \baseapproach (ours)                          & $ \emb{h} \otimes \emb{r} \cdot \emb{t}$                                                       & $\emb{h},\emb{r},\emb{t} \in \Quaternions$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   \approach (ours)                              & $ \ConvolutionWithProjection(\emb{h},\emb{r} ) \circ (\emb{h} \otimes \emb{r}) \cdot \emb{t}$ & $\emb{h},\emb{r},\emb{t} \in \Quaternions$    & BCE & KvsAll  & Adam    & Dropout, BatchNorm \\
   \midrule
   \baseapproachocto (ours)                      & $\emb{h} \bigstar \emb{r} \cdot \emb{t}$                                                                       & $\emb{h},\emb{r},\emb{t} \in \Octonions$      & BCE & KvsAll  & Adam    & Dropout, BatchNorm\\
   \approachocto (ours)                          & $\ConvolutionWithProjection(\emb{h},\emb{r} ) \circ (\emb{h} \bigstar \emb{r} ) \cdot \emb{t}$                 & $\emb{h},\emb{r},\emb{t} \in \Octonions$      & BCE & KvsAll  & Adam    & Dropout, BatchNorm\\
  \bottomrule
\end{tabular}%}
\end{table*}
